Satisfiability of Constrained Horn Clauses on Algebraic Data Types: A Transformation-based Approach

We address the problem of checking the satisfiability of Constrained Horn Clauses (CHCs) defined on Algebraic Data Types (ADTs), such as lists and trees. We propose a new technique for transforming CHCs defined on ADTs into CHCs where the arguments of the predicates have only basic types, such as integers and booleans. Thus, our technique avoids, during satisfiability checking, the explicit use of proof rules based on induction over the ADTs. The main extension over previous techniques for ADT removal is a new transformation rule, called differential replacement, which allows us to introduce auxiliary predicates, whose definitions correspond to lemmas that are used when making inductive proofs. We present an algorithm that performs the automatic removal of ADTs by applying the new rule, together with the traditional folding/unfolding rules. We prove that, under suitable hypotheses, the set of the transformed clauses is satisfiable if and only if so is the set of the original clauses. By an experimental evaluation, we show that the use of the new rule significantly improves the effectiveness of ADT removal. We also show that our approach is competitive with respect to tools that extend CHC solvers with the use of inductive rules.

==> 42_Soundness.tex <==
\newcommand{\Iff}{\leftrightarrow}
\newcommand{\ONLYIF}{\Rightarrow}
\newcommand{\IFF}{\Leftrightarrow}

First, we recall and recast in our framework
some definitions and facts taken from the literature~\cite{EtG96,TaS84,TaS86}.
Besides the rules presented in Section~\ref{subsec:Rules} above,
let us also consider the following rule R8 which, given a transformation sequence 
$P_0 \Rightarrow P_1 \Rightarrow \ldots \Rightarrow P_i$, for some $i\!\geq\!0$, 
allows us to 
extend it by constructing a new set $P_{i+1}$ of CHCs such as $P_i\Rightarrow P_{i+1}$.

\medskip

\hrule
\vspace*{1.5mm}
%
\noindent 
\textbf{(R8)~Goal Replacement Rule.} Let  
$C$:~${H}\leftarrow c, c_{1}, {G}_{L},
{G}_{1}, {G}_{R}$ be a clause in~${P}_{i}$.
If in 
clause~$C$ we  \emph{replace} $c_1,G_1$ by $c_2,G_2$, 
we derive  clause~$D$:
${H}\leftarrow c, c_{2}, {G}_{L},
{G}_{2}, {G}_{R}$, and we get 
$P_{i+1} = ({P}_{i}\setminus\{C\})\cup \{D\}$. 
\smallskip
\hrule

\medskip

Now let us introduce two particular kinds of Goal Replacement Rule: 
(i)~{\it{body weakening}}, and (ii)~{\it{body strengthening}}.
First, for the Goal Replacement Rule, we need to consider the following two tuples of variables:

\vspace*{1mm}
$T_1 = \mathit{vars}(\{c_{1},{G}_{1}\}) 
\setminus \mathit{vars}(\{{H}, c, {G}_{L},{G}_{R}\})$,~~ and

$T_2 = \mathit{vars}(\{c_{2},{G}_{2}\}) 
\setminus \mathit{vars}(\{{H}, c, {G}_{L},{G}_{R}\})$. 
%
%
%

\vspace*{1mm}
\noindent
The Goal Replacement Rule is said to be a {\em body weakening} if the
following two conditions hold:

\vspace*{1mm}

\makebox[12mm][r]{(W.1)~~} $M(\textit{Definite}(P_0)\cup \mathit{Defs}_i) \models \forall\,( c_{1}\! \wedge \! {G}_{1}
\rightarrow \exists T_2.\, c_{2}\! \wedge \! {G}_{2})$

\makebox[12mm][r]{(W.2)~~} $\ell(H)\!>\!\ell(\mathit{A})$, for every atom $A$ occurring 
in $G_2$ and not in $G_1$.

\smallskip
\noindent 
\noindent The Goal Replacement Rule is said to be a \emph{body strengthening} if the
following condition holds:

\vspace*{1mm}
\makebox[12mm][c]{(S)~~} $M(\textit{Definite}(P_0)\cup \mathit{Defs}_i) \models \forall \, (c_{2}\! \wedge \! {G}_{2}
\rightarrow \exists T_1.\, c_{1}\! \wedge \! {G}_{1})$.

\vspace*{1mm}


\smallskip

Usually, in the literature
the Goal Replacement Rule is presented by considering the conjunction 
of Conditions~(W.1) and~(S), thereby considering the quantified equivalence
$\forall \, ( (\exists T_1.\, c_{1}\! \wedge \! {G}_{1})
\Iff (\exists T_2.\, c_{2}\! \wedge \! {G}_{2}))$.
We have split that equivalence into the two associated implications.
This has been done because, 
when proving the Soundness result (see Theorem~\ref{thm:unsat-preserv} in this section) and the Completeness result 
(see Theorem~\ref{thm:sat-preserv}  in Section~\ref{subsec:completeness}),
it is convenient to present %
the preservation
of the least $\mathbb D$-models %
into two parts as specified by the following two theorems.

\begin{theorem}
\label{thm:cons} Let $D_0, \ldots, D_n$ be sets of definite CHCs
and let \mbox{$D_0 \repl \ldots \repl D_n$}
be a transformation sequence constructed using rules
{\rm R1} $($Definition$)$, {\rm R2} $($Unfolding$)$, {\rm R3} $($Folding$)$, and 
{\rm R8} $($Goal Replacement$)$. Suppose that
Condition~{\rm (U)} of Theorem~$\ref{thm:unsat-preserv}$ holds and all 
goal replacements are body weakenings.
%
Then $M({D}_0\cup \mathit{Defs}_n)\subseteq M({D}_n)$.
\end{theorem}

\begin{theorem}
	\label{thm:pc} Let $D_0, \ldots, D_n$ be sets of definite CHCs
	and let \mbox{$D_0 \repl \ldots \repl D_n$}
	be a transformation sequence constructed using rules
	{\rm R1} $($Definition$)$, {\rm R2} $($Unfolding$)$, {\rm R3} $($Folding$)$, and 
	{\rm R8} $($Goal Replacement$)$. Suppose that, for all applications of~{\rm R3}, Condition {\rm (E)} 
	holds $($see Definition~$\ref{def:condR}$ in Section~$\ref{sec:Completeness}$$)$
	and all goal replacements are 
	body strengthenings.
	Then \(M( D_0\cup \mathit{Defs}_n)\supseteq M( D_n) \).
\end{theorem}

For the proof of Theorems~\ref{thm:cons} and~\ref{thm:pc} we refer 
to the results presented in the literature~\cite{EtG96,TaS84,TaS86}.
The correctness of the transformation rules with respect to 
the least Herbrand model semantics has been first proved in the landmark
paper by Tamaki and Sato~\cite{TaS84}.
In a subsequent technical report~\cite{TaS86}, the same authors
extended that result 
by introducing the notion of the {\it level\/} of an atom, 
which we also use in this paper (see the notion defined 
at the beginning of Section~\ref{subsec:Rules}). 

The use of atom levels allows less restrictive 
applicability conditions on the Folding and Goal Replacement Rules.
Later, Etalle and Gabbrielli~\cite{EtG96} extended Tamaki and Sato's results 
to the \mbox{$\mathbb D$-model} semantics of
{\em constraint logic programs} (in the terminology used in
this paper, a constraint logic program is a 
set of definite constrained Horn clauses).

There are three main differences between our presentation of the correctness 
results for the transformation rules with respect to 
the presentation considered in %
%
the literature~\cite{EtG96,TaS84,TaS86}.

First, as already mentioned, we kept the two Conditions~(E) and~(S), 
which guarantee
the inclusion \(M(D_0\!\cup\! \mathit{Defs}_n)\!\supseteq\! M( D_n) \) (called 
{\em Partial Correctness} by Tamaki and Sato~\cite{TaS86}),
separated from the three Conditions~(U), (W.1), and~(W.2), which guarantee
the reverse inclusion \(M(D_0\cup\mathit{Defs}_n)\!\subseteq\! M( D_n) \).
All five conditions together garantee the equality
\(M(D_0\!\cup\! \mathit{Defs}_n)\!=\!M( D_n) \)
(called {\em Total Correctness} by Tamaki and Sato~\cite{TaS86}).


Second, Tamaki and Sato's conditions for the correctness of the Goal Replacement
Rule are actually more general than ours, as they
use a well-founded relation which is based on atom levels and
also on a suitable measure (called \mbox{\em weight-tuple measure}~\cite{TaS86})
of the successful derivations of an 
atom in $M( D_0\cup \mathit{Defs}_n)$. 
Our simpler conditions straightforwardly imply Tamaki and Sato's ones, 
and are sufficient for our purposes in the present paper.

Third, Tamaki and Sato papers~\cite{TaS84,TaS86} 
do not consider constraints, whereas 
Etalle and Gabbrielli results for constraint logic programs do not consider
Goal Replacement~\cite{EtG96}. However, Tamaki and Sato's proofs can easily be 
extended to
constraint logic programs by simply dealing with atomic constraints as atoms
with level 0 and assigning positive levels to all other atoms. 


\medskip

From Theorem~\ref{thm:cons}, we get the following 
Theorem~\ref{thm:unsat},
which relates the satisfiability of sets of clauses obtained 
%
by applying the transformation rules to the satisfiability of the original sets of clauses.

\begin{theorem}
\label{thm:unsat} 
Let $P_0 \repl \ldots \repl P_n$
be a transformation sequence constructed using rules
{\rm R1} $($Definition$)$, {\rm R2} $($Unfolding$)$, {\rm R3} $($Folding$)$, and 
{\rm R8} $($Goal Replacement$)$. Suppose that
Condition~{\rm (U)} of Theorem~$\ref{thm:unsat-preserv}$ holds and all 
goal replacements are body weakenings.
If $P_n$ is satisfiable, then $P_0$ is satisfiable.
\end{theorem}

\begin{proof}
First, we observe that $P_0$ is satisfiable iff 
$P_0 \cup \textit{Defs}_n$ is satisfiable. Indeed, we have that: 
(i)~if~$\mathcal{M}$ is a $\mathbb D$-model of $P_0$, then the $\mathbb D$-interpretation
$\mathcal{M} \cup \{\textit{newp}(a_1,\ldots,a_k) \mid \textit{newp}$ 
is a head predicate
in $\textit{Defs}_n \mbox{ and } a_1,\ldots, a_k$ are ground terms$\}$
is a $\mathbb D$-model of $P_0 \cup \textit{Defs}_n$,
and (ii)~if $\mathcal{M}$ is a $\mathbb D$-model of $P_0 \cup \textit{Defs}_n$, then
all clauses of $P_0$ are true in $\mathcal{M}$, and hence
$\mathcal{M}$  is a $\mathbb D$-model of $P_0$.

Then, let us consider a new transformation 
sequence  $P'_0\Rightarrow \ldots \Rightarrow P'_n$
obtained from the  sequence $P_0\Rightarrow \ldots \Rightarrow P_n$
by replacing each occurrence of \textit{false} in the head of
a clause by a fresh, new predicate symbol, say $f$.
$P'_0,\ldots,P'_n$ are sets of definite clauses, and thus, for $i=0,\ldots,n,$ $\textit{Definite}(P'_i)= P'_i$.
The sequence \mbox{$P'_0\Rightarrow \ldots \Rightarrow P'_n$} satisfies the 
hypotheses of Theorem~\ref{thm:cons}, and hence 
$M(P'_0\cup \mathit{Defs}_n)\!\subseteq M(P'_n)$. We have that:    

\noindent
\makebox[12mm][l]{}$P_n$ is satisfiable

\noindent
\makebox[12mm][l]{implies}{$P'_n\cup \{\neg f\}$ is satisfiable}


\noindent
\makebox[12mm][l]{implies}{$f\not\in M(P'_n)$}

\noindent
\makebox[12mm][l]{implies,}\,by Theorem~\ref{thm:cons}, 
$f\not\in M(P'_0 \cup \textit{Defs}_n)$ 

\noindent
\makebox[12mm][l]{implies}{$P'_0 \cup \textit{Defs}_n\cup \{\neg f\}$ is satisfiable}

\noindent
\makebox[12mm][l]{implies}{$P_0 \cup \textit{Defs}_n$ is satisfiable}

\noindent
\makebox[12mm][l]{implies}{$P_0$ is satisfiable.} \hfill$\Box$
\end{proof}


Now, in order to prove Theorem~\ref{thm:unsat-preserv} of 
Section~\ref{sec:TransfRules}, which states the soundness of rules R1--R7, 
we show that rules R4--R7 are all body weakenings.

\medskip

An application of rule~R4~(Clause Deletion), by which we delete
clause~$C$: $H\leftarrow c,G$, 
whenever the constraint~$c$ is unsatisfiable, is equivalent to
the replacement of the body of clause $C$ by {\it false}. 
Since $c$ is unsatisfiable, we have that:

\smallskip
$M(\textit{Definite}(P_0)\cup \mathit{Defs}_i) \models \forall\,(c \wedge G \rightarrow {\it false})$

\smallskip
\noindent
and Condition (W.1) of rule R8 holds. Also Condition~(W.2), that is:

\vspace*{1mm}
$\ell(H)\!>\!\ell(\mathit{A})$, for every atom $A$ occurring in ${\it false}$ 

\vspace*{1mm}
\noindent
trivially holds, because there are no atoms in ${\it false}$.
Thus, the replacement of the body of clause $H\leftarrow c,G$ by {\it false}
is a body weakening.

\medskip 

Let us now consider rule~R5 (Functionality). 
Let $F(X,Y)$ be a conjunction of atoms 
that defines a functional relation from~$X$ to~$Y$, that is, Property (\textit{Funct})
of Section~\ref{sec:CHCs} holds for $F(X,Y)$.
When rule~R5 is applied whereby a conjunction $F(X,Y),F(X,Z)$
is replaced by the new conjunction $Y\!=\!Z,\ F(X,Y)$, we have that:

\vspace*{1mm}
$M(\mathit{Definite}(P_0)\cup \mathit{Defs}_i) \models \forall(F(X,Y) \wedge F(X,Z) \rightarrow Y\!=\!Z)$

\vspace*{1mm}
\noindent
and hence Condition~(W.1) of rule R8 holds. When this replacement is performed, also Condition~(W.2) trivially holds, and thus
rule~R5 is a body weakening. 

\medskip

An application of rule~R6 (Totality) replaces a conjunction $F(X,Y)$
by {\it true} (that is, the empty conjunction), which is implied by any formula. Hence
{Conditions (W.1) and (W.2) trivially hold,} %
and rule~R6 is a body weakening. 
\medskip

For rule~R7 (Differential Replacement) we prove the following lemma.
Recall that by $F(X;Y)$ we denote a conjunction of atoms 
that defines a total, functional relation from~$X$ to~$Y$.


\begin{lemma}\label{lemma:R7unsat} Let us consider a transformation sequence 
$P_{0}\Rightarrow \ldots \Rightarrow P_{i}$ and a 
clause $C${\rm :}~$H\leftarrow c,  G_L,F(X;Y),G_R$ in $P_{i}$. 
Let us assume that by applying rule~{\rm R7} on clause~$C$ using 
the definition clause

\smallskip
$D{\rm :}~\mathit{diff}(Z) \leftarrow d, F(X;Y), R(V;W),$

\smallskip
\noindent
where\,{\rm :} $(D1)$~$W \cap \vars(C) = \emptyset,$  and
$(D2)$~$\mathbb{D}\models\forall (c\rightarrow d),$ 
we derive clause

\smallskip
$E${\rm :} $H\leftarrow c,  G_L,R(V;W), \mathit{diff}(Z), G_R$

\smallskip
\noindent
and we get the new set 
$P_{i+1} = (P_{i}\setminus\{C\}) \cup \{E \}$ of clauses. Then,

\smallskip
$M(\textit{Definite}(P_0) \cup \mathit{Defs}_i)\models \forall( c \wedge F(X;Y) \rightarrow \exists W.\,(R(V;W) \wedge \mathit{diff}(Z)))$.
\end{lemma}

\begin{proof} Let $\mathcal M$ denote $M(\textit{Definite}(P_0) 
\cup \mathit{Defs}_i)$.
Since, %
$R(V;W)$ is a total, functional conjunction from $V$ to $W$
with respect to~$\textit{Definite}(P_0) \cup  \mathit{Defs}_i$,
we have:

\smallskip

$\mathcal M\models \forall\,( c \wedge F(X;Y) \rightarrow \exists W.\, R(V;W))$ \hfill $(\alpha)$~~~~

\smallskip
\noindent
Since, by Condition~$(D1)$, none of the variables in $W$ occurs in~$C$, from definition~$D$, we get:

\smallskip

$\mathcal M \models \forall\,(d \wedge F(X;Y) \wedge R(V;W) \rightarrow \mathit{diff}(Z))$\hfill $(\beta)$~~~~

   \smallskip

\noindent
From~$(\alpha)$, $(\beta)$, and Condition~$(D2)$, we get the thesis.\hfill $\Box$
\end{proof}

\medskip

From Lemma~\ref{lemma:R7unsat}
it follows that rule~R7, which replaces in the body of 
clause~$C${\rm :} $H\leftarrow c,  G_L,F(X;Y),G_R$
the conjunction~$F(X;Y)$ by the new conjunction $R(V;W)$, $\mathit{diff}(Z)$, 
is a body weakening, assuming that $\ell(H)\!>\!\ell(\mathit{diff}(Z))$.
Recall that, since clause $D$ is a definition clause, we  
have that $\ell(\mathit{diff}(Z))\!\geq\!\ell(\mathit{R})$, and thus we have
that $\ell(H)\!>\!\ell(\mathit{R})$.

The following lemma summarizes the facts we have shown above about rules~R4--R7.

\begin{lemma}\label{lemma:weakening} 
The applications of rules {\rm R4--R7} are all body weakenings.
\end{lemma}

Finally, having proved Lemma~\ref{lemma:weakening}, we can
 present the proof of Theorem~\ref{thm:unsat-preserv}.

\medskip

%
\noindent 
{\it Proof of Theorem~$\ref{thm:unsat-preserv}$}.
Let $P_0 \Rightarrow P_1 \Rightarrow \ldots \Rightarrow P_n$ be 
a transformation sequence constructed using rules {\rm{R1--R7}}. Then,
by Lemma~\ref{lemma:weakening},
that sequence
 can also be constructed by applications of rules {\rm{R1--R3}} together with
applications of rule~R8 which are all body weakenings. 
Since by hypothesis of Theorem~\ref{thm:unsat-preserv}, Condition~(U) does hold,
by applying Theorem~\ref{thm:unsat} we get the thesis.~\hfill~$\Box$
%


==> 7_Experiments_subsects.tex <==
In this section we present the experimental evaluation we have performed
for assessing the effectiveness of our transformation-based CHC %
{satisfiability checking} method.

We have implemented our method %
in a tool called {\sc AdtRem}
and we have compared the results obtained by running our tool with those
obtained by running:
(i) the CVC4 SMT solver~\cite{ReK15} extended with inductive reasoning and lemma
generation,
(ii) the AdtInd solver~\cite{Ya&19}, which makes use of a syntax-guided
synthesis strategy~\cite{Al&13} for lemma generation, and
(iii) the Eldarica CHC solver~\cite{HoR18}, which combines
predicate abstraction~\cite{GrS97} with counterexample-guided
abstraction refinement~\cite{Cl&03}.
{\sc AdtRem} is available at {\small{\url{https://fmlab.unich.it/adtrem/}}}.

%
\subsection{The workflow of the {\sc AdtRem} tool}
\label{subsec:AdtRem-workflow}

Our {\sc AdtRem} tool implements the satisfiability checking method %
presented in Section~\ref{subsec:solvingCHCs} as follows.
First, {\sc AdtRem}
 makes use of the VeriMAP system~\cite{De&14b} to perform the steps
specified by Algorithm~\Diff. It takes as input a
set~$P_0$ of CHCs and, if it terminates, it
 produces as output a set~$P_n$ of CHCs that 
have basic types.
Then, in order to show the satisfiability of $P_{0}$, 
{\sc AdtRem} invokes the Eldarica CHC solver to
show the satisfiability of~$P_n$.

If Eldarica proves that $P_n$ is satisfiable,
then, by the soundness of
the transformation Algoritm~\Diff~(see Theorem~\ref{thm:soundness-AlgorithmR}),
$P_0$ is satisfiable and
{\sc AdtRem} returns the answer `\textit{sat}'.
In particular, the implementation of the \textit{Unfold} procedure
enforces Condition~(U) of
Theorem~\ref{thm:unsat-preserv}, which indeed ensures the 
soundness of Algoritm~\Diff.

If Eldarica proves that $P_n$ is unsatisfiable 
by constructing a counterexample CEX,
{\sc AdtRem} proceeds by checking whether or not Conditions (E)
and (F), which guarantee the completeness of Algoritm~\Diff, hold (see Theorem~\ref{thm:completeness-AlgorithmR}).
In particular, during the execution of Algoritm~\Diff,
{\sc AdtRem} checks Condition (E) when applying the
Folding Rule R3, and Conditions (F2) and (F3) when applying the Differential Replacement Rule~R7.
{\sc AdtRem} marks all clauses in $P_n$ derived by a sequence of transformation 
steps
where one of the Conditions (E), (F2), and (F3) is not satisfied.
%
%
%
%
%
%
%
%
%

Then, {\sc AdtRem} looks at the counterexample CEX constructed by Eldarica
to verify whether or not any instance of the marked clauses is used
for the construction of CEX.
If this is the case, it is not possible to establish the unsatisfiability of
$P_0$ from the unsatisfiability of~$P_n$ (as completeness of 
Algoritm~\Diff~may not hold) and hence {\sc AdtRem} returns
the answer `\textit{unknown}' as the result of the satisfiability 
check for $P_{0}$.
%

Otherwise, if {no instance of a marked clause}
is used in CEX, then {\sc AdtRem} proceeds by checking
Condition~(F1) of Definition~\ref{def:condF}. 
%
%
%
%
{Recall that, by Proposition~\ref{prop:fun-preserv}, Condition~(F1) can be checked 
by inspecting the clauses defining the differential 
predicates in $\textit{Definite}(P_n)$.}
To perform this check,
for each differential predicate $\textit{diff}_k$ introduced by 
Algorithm~\Diff~and occurring in CEX, {\sc AdtRem}
produces {a clause, call it $\textit{fun-diff}_k$,} of the
form:
%
%
%
%
%
%

\smallskip

$~\textit{false}\leftarrow$ $O_1\!\neq\!O_2,$ 
$\textit{diff}_k(I,O_1), \textit{diff}_k(I,O_2)$

\smallskip

\noindent
where $I$ and $O_i$, for $i=1,2,$ are the tuples of input and output
variables, respectively, of $\textit{diff}_k(I,O_i)$.
Then, {\sc AdtRem} runs Eldarica to check the satisfiability
of $\bigcup_k\{\textit{fun-diff}_k\}\cup D_n$,
where $D_n$ is the set of clauses defining $\textit{diff}_k$ in
$\textit{Definite}(P_n)$ (see Example~\ref{ex:func}).
Now, this satisfiability check may succeed (Case 1) or may not succeed (Case 2).
In Case 1, 
%
Condition~(F1) holds and, by the completeness of 
Algorithm~\Diff~(see Theorem~\ref{thm:completeness-AlgorithmR}), 
we have that $P_0$ is %
unsatisfiable and {\sc AdtRem} returns the answer `\textit{unsat}'. 
%
%
%
%
In Case 2, Condition~(F1) cannot be shown,
and {\sc AdtRem} returns the answer `\textit{unknown}' as the result of the
satisfiability of~$P_{0}$.
%
%
%

%
\subsection{Benchmark suite}
Our benchmark suite consists of 251 {verification} %
problems over inductively
defined data structures, such as lists, queues, heaps, and trees.
Out of these 251 problems, 168 of them
 refer to properties that hold (\textit{valid}
properties) and the remaining 83 refer to properties that do not hold
(\textit{invalid} properties).

The 168 problems specifying valid properties have been adapted from the
benchmark suite considered by Reynolds and Kuncak~\cite{ReK15}, and
originate from benchmarks used by various theorem provers, such as
CLAM~\cite{IrB96}, HipSpec~\cite{Cl&13}, IsaPlanner~\cite{DiF03,Jo&10},
and Leon~\cite{Su&11}.
In particular, we have considered Reynolds and Kuncak's `dtt'
encoding where natural numbers are represented using the built-in
SMT type {\it Int}.
From those problems we have discarded:
(i)~the ones that do not use ADTs, and
(ii)~the ones that cannot be directly represented in Horn clause format.
In order to make a comparison between our approach and Reynolds-Kuncak's
one on a level playing field, since {\sc AdtRem} supports neither higher
order functions nor user-provided lemmas,
(i)~we have replaced higher order functions by suitable first order instances,
and
(ii)~we have removed all auxiliary lemmas from the formalization of the  
%
problems.
We have also used LIA constraints, instead of the basic functions recursively
defined over natural numbers, such as the {\it plus} function and
{\it less-or-equal} relation, so that the solver can deal with them by using
the LIA theory.

The 83 problems specifying invalid properties have been obtained from those
specifying valid properties by either negating the properties or
modifying {the definitions} of 
the predicates on which the properties depend.

The benchmark suite is available at {\small{\url{https://fmlab.unich.it/adtrem/}}}.

%
\subsection{Experiments}

We have performed the following experiments.

\smallskip

\noindent\hangindent=4mm
1. We have run the `cvc4+ig' configuration of the CVC4 solver extended
with inductive reasoning and also the AdtInd solver on the 251 
{verification} %
problems in SMT-LIB format.

\noindent\hangindent=4mm
2. Then, we have translated each {verification} %
problem into
a set, call it $P_0$, of CHCs in the Prolog-like syntax supported by {\sc AdtRem} by using a
modified version of the SMT-LIB parser of the ProB system~\cite{LeB03}.
We have run Eldarica {v2.0.5}, which uses no induction-based
mechanism for handling ADTs, to check the satisfiability of the
SMT-LIB translation of $P_0$\footnote{We have also performed analogous experiments on the set of valid
properties by using Z3-SPACER~\cite{Ko&13}, instead of Eldarica,
as reported on an earlier version of this paper~\cite{De&20a}.
The results of those experiments, which we do not report here,
are very similar to those shown in	Table~\ref{tab:Exper-Results}.}\!.
%
%
%
%

\noindent\hangindent=4mm
3. Finally, we have run {\sc AdtRem} to check the satisfiability %
of $P_0$.
If {\sc AdtRem} returns `\textit{sat}', the property specified by $P_0$ 
is reported to be valid.
If {\sc AdtRem} returns `\textit{unsat}', the property is reported to be invalid.
%
%



\smallskip
\noindent
Experiments have been performed 
on an Intel Xeon CPU E5-2640 2.00GHz with 64GB RAM under CentOS
and for each problem we have set a timeout limit of 300 seconds.


